Adaptive stochastic Galerkin FEM for lognormal coefficients in hierarchical tensor representations

Stochastic Galerkin methods for non-affine coefficient representations are known to cause major difficulties from theoretical and numerical points of view. In this work, an adaptive Galerkin FE method for linear parametric PDEs with lognormal coefficients discretized in Hermite chaos polynomials is derived. It employs problem-adapted function spaces to ensure solvability of the variational formulation. The inherently high computational complexity of the parametric operator is made tractable by using hierarchical tensor representations. For this, a new tensor train format of the lognormal coefficient is derived and verified numerically. The central novelty is the derivation of a reliable residual-based a posteriori error estimator. This can be regarded as a unique feature of stochastic Galerkin methods. It allows for an adaptive algorithm to steer the refinements of the physical mesh and the anisotropic Wiener chaos polynomial degrees. For the evaluation of the error estimator to become feasible, a numerically efficient tensor format discretization is developed. Benchmark examples with unbounded lognormal coefficient fields illustrate the performance of the proposed Galerkin discretization and the fully adaptive algorithm.

==> pgfplotsoptions.tex <==
%% create a new cycle list for egsz plots
\pgfplotscreateplotcyclelist{egsz color}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=square*},
  {brown!60!black,every mark/.append style={fill=brown!90!black},mark=otimes*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=diamond*},
}

\pgfplotscreateplotcyclelist{egsz color twocol}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=*},
  {blue!60!black, every mark/.append style={fill=blue!80!black!30}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=diamond*},
  {red!60!black,  every mark/.append style={fill=red!80!black!30},  mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=triangle*},
  {green!30!black,every mark/.append style={fill=green!70!black!30},mark=triangle*},
}
  
\pgfplotscreateplotcyclelist{egsz bw twocol}{%
  {black, every mark/.append style={fill=black},    mark=*},
  {black, every mark/.append style={fill=black!15}, mark=*},
  {black,  every mark/.append style={fill=black},     mark=diamond*},
  {black,  every mark/.append style={fill=black!15},  mark=diamond*},
  {black,every mark/.append style={fill=black},   mark=triangle*},
  {black,every mark/.append style={fill=black!15},mark=triangle*},
}
  
\pgfplotscreateplotcyclelist{egsz color threecol}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=diamond*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=diamond*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=triangle*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=triangle*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=triangle*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=square*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=square*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=square*},
  }

\pgfplotscreateplotcyclelist{egsz bw threecol}{%
  {black, every mark/.append style={fill=black},    mark=*},
  {black, every mark/.append style={fill=black!35}, mark=*},
  {black, every mark/.append style={fill=black!5}, mark=*},
  {black,  every mark/.append style={fill=black},     mark=diamond*},
  {black,  every mark/.append style={fill=black!35},  mark=diamond*},
  {black,  every mark/.append style={fill=black!5},  mark=diamond*},
  {black,every mark/.append style={fill=black},   mark=triangle*},
  {black,every mark/.append style={fill=black!35},mark=triangle*},
  {black,every mark/.append style={fill=black!5},mark=triangle*},
  {black,every mark/.append style={fill=black},   mark=square*},
  {black,every mark/.append style={fill=black!35},mark=square*},
  {black,every mark/.append style={fill=black!5},mark=square*},
}  
  
\pgfplotscreateplotcyclelist{egsz color comparison}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black!50}, mark=square*},
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=triangle*},
}

\pgfplotscreateplotcyclelist{egsz color mi}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=square*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=diamond*},
}

\pgfplotscreateplotcyclelist{egsz bw mi}{%
  {black, every mark/.append style={fill=black}, mark=*},
  {black,  every mark/.append style={fill=black!35},  mark=square*},
  {black,every mark/.append style={fill=black!5},mark=diamond*},
}

%% set styles for general plots and error plots
\pgfplotsset{
  /tikz/tikzpic options/.style={
    scale=0.8,
  },
  egsz plot/.style={
    thin, % very thin, thin, semithick, thick, very thick
    %rounded corners=3pt,
    label style={font=\footnotesize}, %\tiny, \scriptsize, \footnotesize
    width=0.65\textwidth,
    height=0.3\textheight,
    grid=major, % none, major, minor, both
    legend columns=1,
    legend pos=south west,
    legend style={font=\tiny, rounded corners=2pt, cells={anchor=west}},
  },
  dof plot/.style={
    egsz plot,
    xlabel=TTdofs,
    xlabel style={yshift=0.5em},
  },
  %
  right side/.style={
    ylabel=,
  },
  %
  top label/.style={
    legend pos=north west,
  },
  %
  wide label/.style={
    legend columns=3,
  },
  sol error plot/.style={
  dof plot,
  cycle list name=egsz bw twocol,
  ylabel=relative root mean square error,
  },
  %
  sol error plot dbl 1/.style={
  dof plot,
  width = 0.48\textwidth,
  cycle list name=egsz bw twocol,
  ylabel=relative root mean square error,
  },
  sol error plot dbl 2/.style={
  dof plot,
  width = 0.48\textwidth,
  cycle list name=egsz bw twocol,
  ylabel=,
  },
  %
  estimator efficiency plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=energy error,
    ylabel style={yshift=-1.9ex,xshift=1em},
  },
  estimator efficiency plotb/.style={
    dof plot,
    cycle list name=egsz bw threecol,
    legend columns=3,
    ylabel=efficiency index,
    ylabel style={yshift=-1.9ex,xshift=1em},
    legend to name=efflegend,
    mark options={scale=0.75},
    legend style={mark options={scale=0.75}},
  },
  estimator efficiency plotc/.style={
    estimator efficiency plot,
    legend pos=north west,
  },
  %
  error multiindex plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=energy error (multi-indices),
    ylabel style={yshift=-1.9ex,xshift=1em},
  },
  %
  cells multiindex plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=cells/multi-indices,
    ylabel style={yshift=-1.9ex,xshift=1em},
    legend pos=north west,
  },
  %
  error comparison plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=energy error,
    ylabel style={yshift=-1.9ex,xshift=1em},
  },
  %
  mi error plot/.style={
    dof plot,
    cycle list name=egsz bw mi,
    ylabel=number multi-indices,
    ylabel style={yshift=-1.9ex,xshift=1em},
    xlabel=energy error,
    legend pos=north east,
    legend columns=1,
  },
  estimator comparison plot/.style={
    dof plot,
    width=0.45\textwidth,
    legend columns=3,
    cycle list name=egsz bw threecol,
    ylabel=,
    ylabel style={yshift=-1.9ex,xshift=1em},
    legend to name=legend,
    mark options={scale=0.75},
    legend style={mark options={scale=0.75}},
  },
}

\tikzset{slopetriangle/.style={
    bottom color=black!20,
    middle color=black!5,
    top color=white,
    draw=black}
    }

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> tttreatment.tex <==
\section{Solution of the discrete problem in TT format}
\label{sec:ALS}

The fully discretized problem can be solved easily in the TT format using the \emph{Alternating Least Squares (ALS)} algorithm as introduced in \cite{EPS}. Other algorithms like Riemannian optimization are also feasible~\cite{Absil2008,Kressner2014}.

We precondition the ALS algorithm using the mean of the discretized coefficient $a_{\Delta,s}$:
\begin{align}
\bar a(x) &:= \mathbb E(a_{\Delta,s}(x,\cdot)) = \int_\Gamma a_{\Delta,s}(x,y) \dgamthrh{y} \\
&= \sum_{k_1=1}^{s_1} \cdots \sum_{k_L=1}^{s_L} a_0[k_1](x) \prod_{\ell=1}^L \sum_{\nu_\ell =0}^{q_\ell-1} A_\ell(k_\ell,\nu_\ell,k_{\ell+1}) \int_{\mathbb R} \Hthrh_{\nu_\ell}(y_\ell) \dx{\gamma_{\theta\rho,m}}(y_\ell) \\
&= \sum_{k_1=1}^{s_1} \cdots \sum_{k_L=1}^{s_L} a_0[k_1](x) \prod_{\ell=1}^L A_\ell(k_\ell,0,k_{\ell+1}).
\end{align}
This holds since
\begin{equation}
\int_{\mathbb R} \Hthrh_{\nu_\ell}(y_\ell) \dx{\gamma_{\theta\rho,\ell}}(y_\ell) = \delta_{0\nu_\ell}.
\end{equation}
Define $\bar A \in \mathbb R^{N \times N}$ by
\begin{equation}
\bar A(i,j) := \int_D \bar a(x) \nabla \phi_i(x) \cdot \nabla \phi_j(x) \dx{x} \qquad \text{for all } i,j = 1,\ldots,N.
\end{equation}
Then, the mean preconditioner becomes
\begin{equation}
\bar {\mathbf A} := \bar A \otimes I \otimes \ldots \otimes I. 
\end{equation}
The preconditioning procedure is done in the same way as in \cite{EPS}.
\todo{\tiny is it??? I don't know what Manuel is doing there now, but that was the plan.}
